ResolverFuzz: Automated Discovery of DNS Resolver Vulnerabilities with Query-Response Fuzzing

Domain Name System (DNS) is a critical component of the Internet. DNS resolvers, which act as the cache between DNS clients and DNS nameservers, are the central piece of the DNS infrastructure, essential to the scalability of DNS. However, finding the resolver vulnerabilities is non-trivial, and this problem is not well addressed by the existing tools. To list a few reasons, first, most of the known resolver vulnerabilities are non-crash bugs that cannot be directly detected by the existing oracles (or sanitizers). Second, there lacks rigorous specifications to be used as references to classify a test case as a resolver bug. Third, DNS resolvers are stateful, and stateful fuzzing is still challenging due to the large input space. In this paper, we present a new fuzzing system termed ResolverFuzz to address the aforementioned challenges related to DNS resolvers, with a suite of new techniques being developed. First, ResolverFuzz performs constrained stateful fuzzing by focusing on the short query-response sequence, which has been demonstrated as the most effective way to find resolver bugs, based on our study of the published DNS CVEs. Second, to generate test cases that are more likely to trigger resolver bugs, we combine probabilistic context-free grammar (PCFG) based input generation with byte-level mutation for both queries and responses. Third, we leverage differential testing and clustering to identify non-crash bugs like cache poisoning bugs. We evaluated ResolverFuzz against 6 mainstream DNS software under 4 resolver modes. Overall, we identify 23 vulnerabilities that can result in cache poisoning, resource consumption, and crash attacks. After responsible disclosure, 19 of them have been confirmed or fixed, and 15 CVE numbers have been assigned.

==> figures/clustering_performance/clustering_performance.tex <==
\begin{figure*}[t]
	\centering
	\subfigcapskip=-1.5mm
	\subfigure[]{
		\begin{minipage}[t]{0.45\linewidth}
		    \centering
			\includegraphics[width=\linewidth]{figures/clustering_performance/Recur_only.pdf}
		\end{minipage}
		\label{fig:cluster_perf_recur}
	}
    \hspace{-3mm}
    \subfigure[]{
		\begin{minipage}[t]{0.45\linewidth}
		    \centering
			\includegraphics[width=\linewidth]{figures/clustering_performance/Fwd_only.pdf}
		\end{minipage}
		\label{fig:cluster_perf_fwd_only}
	}
	\\
    % \vspace{-1.25mm}
    \subfigure[]{
		\begin{minipage}[t]{0.45\linewidth}
		    \centering
			\includegraphics[width=\linewidth]{figures/clustering_performance/CDNS_w_fb.pdf}
		\end{minipage}
		\label{fig:cluster_perf_cdns_w_fb}
	}
	\hspace{-3mm}
    \subfigure[]{
		\begin{minipage}[t]{0.45\linewidth}
		    \centering
			\includegraphics[width=\linewidth]{figures/clustering_performance/CDNS_wo_fb.pdf}
		\end{minipage}
		\label{fig:cluster_perf_cdns_wo_fb}
	}
	\caption{
        \revise{Number of different vulnerabilities appeared with regard to time in a) recursive-only, b) forward-only, 3) CDNS with fallback and d) CDNS without fallback. Each curve represents one cluster. Each point represents the time when a new vulnerability is triggered in the related cluster.}
        }
	\vspace{-3mm}
	\label{fig:cluster_perf}
\end{figure*}

==> figures/k_means.tex <==
\begin{figure}[t]	
    \centering
    \includegraphics[width=\columnwidth]{figures/k_means_fig.pdf}
    % \vspace{-4mm}
    \caption{SSE (Sum of Squared Error) distribution to different K for bisecting K-means in cache oracle. 
    }
    % \vspace{-2mm}
    \label{fig:k_means}
\end{figure}

==> lists/cfg/cfg_query_partial.tex <==
\lstdefinelanguage{BNF}{
    basicstyle=\ttfamily\footnotesize,
    keywordstyle=\bfseries\footnotesize,
    morekeywords={start, query, Header, Question, QNAME, QTYPE, QCLASS},
    morecomment=[l]{//},
    morekeywords={::=},
    sensitive=true,
    breaklines=true,
        columns=flexible, 
    captionpos=b, 
    frame=tb,
    literate={->}{{$\rightarrow$}}1
          {<}{{\textbf{$\langle$}}}1
          {>}{{\textbf{$\rangle$}}}1
}

\begin{lstlisting}[language=BNF, float, floatplacement=t, caption={Example partial PCFG for DNS query.}, label=lis:cfg_query_partial]
<start> ::= <query>
<query> ::= <Header><Question>
(..truncated..)
<Question> ::= <QNAME><QTYPE><QCLASS>
<QNAME> ::= (base domain)[.40] | 
            (sub-domain)[.40] | 
            (2-9th sub-domain)[.10] | 
            (10-max sub-domain)[.10] |
<QTYPE> ::= A | NS | CNAME | SOA | PTR ...
<QCLASS> ::= IN
\end{lstlisting}


==> lists/cfg/cfg_response_partial.tex <==
\lstdefinelanguage{BNF}{
    basicstyle=\ttfamily\footnotesize,
    keywordstyle=\bfseries\footnotesize,
    morekeywords={start, response, Header, Question, Answer, Authority, Additional, Record, NAME, TYPE, CLASS, TTL, RDLENGTH, RDATA, DOMAIN, IP},
    morekeywords={::=},
    morecomment=[l]{//},
    sensitive=true,
    breaklines=true,
    captionpos=b,
    frame=tb, 
    literate={->}{{$\rightarrow$}}1
          {<}{{\textbf{$\langle$}}}1
          {>}{{\textbf{$\rangle$}}}1
}

\begin{lstlisting}[language=BNF, columns=flexible, float, floatplacement=t, caption={Example partial PCFG for DNS responses.}, label=lis:cfg_response_partial]
<start> ::= <response>
<response> ::= <Header><Answer>
                <Authority><Additional>
(..truncated..)
<Answer> ::= "" | <Record> | <Record>*2 | <Record>*3 | <Record>*4 | <Record>*5
<Record> ::= <NAME><TYPE><CLASS><TTL><RDLENGTH><RDATA>
<NAME> ::= (domain queried)[.2] | 
            (sub-domain)[.2] | 
            (same-level domain)[.2] | 
            (parent domain)[.2] | 
            (unrelated domain)[.2]
<TYPE> ::= (TYPE queried)[.50] | A[.05] | CNAME[.05] | SOA[.05] | PTR[.05] | MX[.05] | TXT[.05] | AAAA[.05] | RRSIG[.05] | SPF[.05]
<CLASS> ::= IN
<TTL> ::= 60
<RDLENGTH> ::= (length of <RDATA>)[.90] |  (random value in [length, 2*length])[.05] |  (random value in [0, length])[.05] 
<RDATA> ::= (randomly generated data decided by <TYPE>)
(..truncated..)
\end{lstlisting}


==> package.tex <==
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
\RequirePackage[normalem]{ulem}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
\providecommand{\DIFmodbegin}{}
\providecommand{\DIFmodend}{}
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
\RequirePackage{listings}
\RequirePackage{color}
\lstdefinelanguage{DIFcode}{
  moredelim=[il][\color{red}\sout]{\%DIF\ <\ },
  moredelim=[il][\color{blue}\uwave]{\%DIF\ >\ }
}
\lstdefinestyle{DIFverbatimstyle}{
	language=DIFcode,
	basicstyle=\ttfamily,
	columns=fullflexible,
	keepspaces=true
}
\lstnewenvironment{DIFverbatim}{\lstset{style=DIFverbatimstyle}}{}
\lstnewenvironment{DIFverbatim*}{\lstset{style=DIFverbatimstyle,showspaces=true}}{}


% some error
\microtypecontext{spacing=nonfrench}


% figure
\usepackage{graphicx}
\usepackage{subfigure}


% ticks and cross marks
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{pslatex}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\definecolor{redx}{RGB}{180,0,0}
\definecolor{greenx}{RGB}{0,180,0}
\newcommand{\redcmark}{\color{redx}\ding{51}}
\newcommand{\greenxmark}{\color{greenx}\ding{55}}
\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}


% reference
\usepackage{cleveref}
\crefname{section}{Section}{Sections}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{equation}{Equation}{equations}
\crefname{algocf}{Algorithm}{algorithms}
\crefname{appendix}{Appendix}{appendices}


% table
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{threeparttable}


% alignment for URL
\def\UrlBreaks{%
  \do\/%
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l%
     \do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z%
  \do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L%
     \do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X\do\Y\do\Z%
  \do0\do1\do2\do3\do4\do5\do6\do7\do8\do9\do=\do/\do.\do:%
  \do\*\do\-\do\~\do\'\do\"\do\-}
\Urlmuskip=0mu plus 0.1mu


% box
\usepackage{tcolorbox}


% check
\usepackage{bbding}


% list
\usepackage{enumerate}
\usepackage{enumitem}


% algorithm
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother


% no indent for footnote
\usepackage[hang,flushmargin]{footmisc}


% compress references
% \usepackage[numbers,sort,compress]{natbib}
% \setlength{\bibsep}{5pt}


% Corresponding author
\usepackage[misc]{ifsym}
\let\Square\relax
% \usepackage{bbding}



==> tables/efficiency/efficiency.tex <==
\begin{table}[t]
  \centering
  \caption{Runtime performance of 4 modes. We run 25 units concurrently on all modes for the maximized throughput.}
  \setlength{\tabcolsep}{4.9pt}
  \begin{threeparttable}  
    \begin{tabular}{c|c|c}
    \toprule
    \textbf{Mode}  & \multicolumn{1}{l|}{\textbf{\# Test cases}} & \multicolumn{1}{l}{\textbf{Throughput (QPS)}} \\
    \midrule
        \textit{Recursive-only} & 187.2K & 2.675 \\
        \textit{Forwarder-only} & 180K  & 2.684 \\
        \textit{CDNS w/o f.b.}\tnote{1} & 180.9K & 2.765 \\
        \textit{CDNS w/\ \ \ f.b.}\tnote{2} & 180.15K & 5.603 \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \footnotesize
      \item \tnote{1}: \textit{CDNS without fallback}. \tnote{2}: \textit{CDNS with fallback}.
    \end{tablenotes}
    \end{threeparttable}
    \vspace{-5mm}
  \label{tab:performance}%
\end{table}%

